Analyzing the Impact of Covid-19 Control Policies on Campus Occupancy and Mobility via Passive WiFi Sensing

Mobile sensing has played a key role in providing digital solutions to aid with COVID-19 containment policies. These solutions include, among other efforts, enforcing social distancing and monitoring crowd movements in indoor spaces. However, such solutions may not be effective without mass adoption. As more and more countries reopen from lockdowns, there remains a pressing need to minimize crowd movements and interactions, particularly in enclosed spaces. This paper conjectures that analyzing user occupancy and mobility via deployed WiFi infrastructure can help institutions monitor and maintain safety compliance according to the public health guidelines. Using smartphones as a proxy for user location, our analysis demonstrates how coarse-grained WiFi data can sufficiently reflect indoor occupancy spectrum when different COVID-19 policies were enacted. Our work analyzes staff and students' mobility data from three different university campuses. Two of these campuses are in Singapore, and the third is in the Northeastern United States. Our results show that online learning, split-team, and other space management policies effectively lower occupancy. However, they do not change the mobility for individuals transitioning between spaces. We demonstrate how this data source can be put to practical application for institutional crowd control and discuss the implications of our findings for policy-making.

==> backup.tex <==

\review{Overall, the reopening of amenities and communal areas within the universities are introduced in stages. For example, while classes are prioritized to revert to on-campus instructions, the utilization of communal areas such as indoor gyms, libraries, cafeterias, common study areas, and lounges continues to limit crowd size [X]. Our analyses have demonstrated the changing occupancy in such areas over different \virus phases (see Figure \ref{fig:schoolAreas}) through our CMS, and it remains relevant in reporting occupancy rates on a more refined time granularity of per hour and per day.} 

\review{Figure \ref{fig:dashboard} visualizes the occupancy rate derived by each WiFi AP on each floor per building within the \amherst university. Operations management officials can select a building and its respective floor to narrow down monitoring to a specific area (e.g., an open study area); see Filter 1 and 2 under \viruss: Building/Floor Selector pane. As explained in Section \ref{sec:inferMeasure}, we used the number of unique MAC addresses seen by our WiFi network (devices) to calculate occupancy percentages (see Pane 3 and 4). The ability to refine our monitoring results from per building to areas per floor can quickly help officials determine areas that may violate zone restrictions. For example, as per Pane 5 and 6, the occupancy heatmaps for each area within the building show a relatively high occupancy rate (in orange) for five areas throughout the day. Note: each area is represented as a row in the y-axis, while the x-axis denotes the time of day.}



From an operational perspective, this analysis can help make informed decisions to actively revise the restricted capacity based on the severity of an outbreak. Instead of a complete shutdown, other workplace policies can be introduced to implement stricter safety measures. One policy is deploying safety ambassadors to regulate social distancing and face-covering among occupants on-ground \cite{X}.\\

%Column: Chicago’s new ‘social distancing ambassadors’ are helping us stay safe

\subsubsection{Online Monitoring Platform} 
Figure \ref{fig:dashboard} displays a dashboard visualizing WiFi data of \amherst university at an aggregated scale, designed for authorized officials as the primary user. The occupancy dashboard displays occupancy percentages derived by each AP on each floor per building.

An authorized official can select a building and its respective floor to narrow down monitoring to a specific zone or a collection of rooms (see Filter 1 and 2 under \viruss: Building/Floor Selector pane). As explained in Section \ref{sec:inferMeasure}, we used the number of unique MAC addresses seen by our WiFi network (devices) to calculate occupancy percentages. The visualization is split into `device-normal' and `device-target'. `device-normal' denotes the actual occupancy percentage for a dedicated area, and `device-target' plots the occupancy exceeding a restricted capacity (i.e., to be determined by safety compliance guidelines). The middle panes display occupancy percentage for each floor per building, while the bottom panes displays occupancy per AP. The ability to refine our monitoring results from building to floor to AP helps an authorized official to determine areas corresponding to the AP that may violate zone restrictions.



\subsubsection{\virus response compliance management} As institutions seek to re-open in the coming semesters, they must fully implement the required \virus protocol and maintain campus operations with as much safety as possible for staff and students. Recall, our tool plots occupancy density exceeding a restricted capacity, which ideally must be up-to-date with current safety compliance guidelines. Once the occupancy threshold is determined, authorized officials can swiftly filter buildings and floors to single out high foot traffic areas. Figure \ref{fig:dashboard2} is a sample dashboard, displaying all relevant information to the target location (nearby APs define the target location). Occupancy density is visualized in the form of a heatmap, with red shade indicating occupancy density over the restricted threshold.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.76\textwidth]{images/dormdashboard.png}
    \caption{Online dashboard for \nus campus displaying occupancy density across different on-campus dormitories and occupancy trends per building throughout several days.}
    \label{fig:dormdashboard}
\end{figure}

At the present day, our three universities have dedicated efforts to employ the WiFi network for \viruss. Figure \ref{fig:dormdashboard} presents an online dashboard for \nuss, centering on all its on-campus dormitories. Having monitoring capabilities on these facilities is especially critical since several dormitory blocks (D1-D3) were repurposed for quarantine use. As reported in Section 4.4, our analysis found the daily occupancy level in dormitories to be approximately 700 every day during the \virus phases. Unexpected occupancy surges in dorms D5 to D10, for example, is when an on-site inspection by safety personnel is warranted.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.76\textwidth]{images/canteendashboard.png}
    \caption{Online dashboard for \smu campus displaying a heat map of occupancy density across different areas in a building throughout different times of the day.}
    \label{fig:canteendashboard}
\end{figure}

Similarly, Figure \ref{fig:canteendashboard} shows an online dashboard for the \smu campus. This visualization is presented to the room detail, concentrating on specific areas of a floor plan. In this example, we show Basement 1 (B1) of Building 7. Note we mentioned in Section \ref{sec:inferMeasure} that Building 7 typically receives high foot traffic as B1 (specifically Area K) is where the main university dining hall is situated. We would expect close to no movements in the building with Area K closed during the lockdown period. However, we can determine a nearby area, Area T (at 9:12 AM), to receive high foot traffic. A fundamental step in preventing \virus is the act of social distancing. Our information can help institutions make more informed decisions, particularly in operations scheduling, to deploy social distancing officers to appropriate zones. 

\subsubsection{Privacy Safeguards} Refer to Figure \ref{fig:dashboard2}, note that users' information connected to the AP is available (bottom left pane); however, these users are anonymized from hashing. We had discussed in Section \ref{sec:privacyEthicalConsiderations} of the privacy safeguards in the event an area is determined to be at high-risk of \virus spread, and digital contract tracing may need to be performed. One viable safeguard is implementing authorization to export the anonymized user list in a .CSV file. Another possibility is to perform de-anonymization separately from the platform, nevertheless requiring appropriate permissions. 

Overall, we believe passive WiFi-sensing is a promising technique to pursue \virus response on a larger scale. We are already providing updates at \smu to the campus facilities managers and the deans of students at \nus regarding the occupancy and mobility levels across the buildings and dorms at each campus.


%Finally, the analysis is a bit coarse grained to actually get useful insights from the study. Looking at more finerdetails or at least some mention of these could add to the overall contribution. For instance, recreational locationas the authors mention could be the gym, or could be some activity (or game), in the former case, gym canbe considered more towards fitness while the latter is more recreational or for relaxation. 

%Overall, we believe this is a very promising avenue to pursue and the administrators at all three universities agree. We are already providing updates at \smu to the campus facilities managers and the deans of students at \nus about the occupancy and mobility levels across the buildings and dorms at each campus.}

==> related.tex <==
\section{Related Work}
\label{sec:related}
Our goal is to enable institutional crowd control and inform policy makers about the effect of various \virus related decisions. This is particularly important as every country is enacting a slew of policies that they believe are best for them~\cite{ILO}. But how do you know if these policies are effective? To help, there have been several online \virus trackers that show the number of infections per country~\cite{worldometer,WHO_Stats,coronatracker,covid_JHU}. Much research also focused on the rate of spread in China~\cite{surveillances2020epidemiological}, possible ways to exit lockdown across the world~\cite{yap2020covid} and campus behaviour in Italy~\cite{Favale_2020}. 

\textcolor{black}{One of the earliest analysis using location data investigated the} cluster of \virus cases in office block in South Korea ~\cite{park2020coronavirus}. \textcolor{black}{Confirmed case-patients supplied their mobile phone location data and were notified of the nearest screening center to get tested. Mobile phones quickly became key for exposure notifications \cite{badr2020association,lee2020testing,dar2020applicability} and safety guidelines \cite{WHO_covid}. For example, Singapore mandated mobile check-ins at public spaces \cite{safeentry} and released the first nationwide Bluetooth-enabled app in the world for its government to trace users in close proximity with a case-patient \cite{tracetogether}. While these apps are essentially for contact tracing, they provide essential information for the municipality to enact appropriate safety policies. Further, mandating any kind of \virus surveillance is more likely to receive strong pushback among democratic communities. It remains necessary to discover approaches for large-scale sensing that  preserve privacy while simultaneously providing multiple communal benefits.}

This analysis is inspired by prior work that uses WiFi data to analyze and understand different settings, which include analyzing the flow of people through buildings \cite{trivedi2020empirical}, how people move in groups \cite{sen2014grumon,jayarajah2015need}, shopper behaviour \cite{hwang2017process}, and even the psychological state of individuals~\cite{zakaria2019stressmon}. These works are on the basis that mobile phone connection to a WiFi access point represents a real-time proxy of user moving on-premise. Hence, we adopt similar techniques and apply it to understand the occupancy and mobility patterns of users. We add to this growing body of work by providing detailed analysis using data from three different campuses (two of which are quite large) that shows the clear effect that various policies have, over two months, on the occupancy and mobility at these campuses. 

 
